Search for new light gauge bosons in Higgs boson decays to four-lepton final states in $pp$ collisions at $\sqrt{s}=8$ TeV with the ATLAS detector at the LHC

This paper presents a search for Higgs bosons decaying to four leptons, either electrons or muons, via one or two light exotic gauge bosons $Z_d$, $H\to Z Z_d \to 4\ell$ or $H\to Z_d Z_d \to 4\ell$. The search was performed using $pp$ collision data corresponding to an integrated luminosity of about 20 fb$^{-1}$ at the center-of-mass energy of $\sqrt{s}=8 $TeV recorded with the ATLAS detector at the Large Hadron Collider. The observed data are well described by the Standard Model prediction. Upper bounds on the branching ratio of $H\to Z Z_d \to 4\ell$ and on the kinetic mixing parameter between the $Z_d$ and the Standard Model hypercharge gauge boson are set in the range $(1$--$9)\times10^{-5}$ and $(4$--$17)\times10^{-2}$ respectively, at 95% confidence level assuming the Standard Model branching ratio of $H\to Z Z^* \to 4\ell$, for $Z_d$ masses between 15 and 55 GeV. Upper bounds on the effective mass mixing parameter between the $Z$ and the $Z_d$ are also set using the branching ratio limits in the $H \to ZZ_d\to 4\ell$ search, and are in the range $(1.5$--$8.7)\times 10^{-4}$ for $15<m_{Z_d} < 35$ GeV. Upper bounds on the branching ratio of $H\rightarrow Z_dZ_d \to 4\ell$ and on Higgs portal coupling parameter, controlling the strength of the coupling of the Higgs boson to dark vector bosons, are set in the range $(2$--$3)\times10^{-5}$ and $(1$--$10)\times 10^{-4}$ respectively, at 95% confidence level assuming the Standard Model Higgs boson production cross sections, for $Z_d$ masses between 15 and 60 GeV.

==> Acknowledgements.tex <==
\section*{Acknowledgments}

% Acknowledgements for papers with collision data
% Version 23-Mar-2015

% Standard acknowledgements start here
%----------------------------------------------

We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC,
Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP,
Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC,
China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic;
DNRF, DNSRC and Lundbeck Foundation, Denmark; EPLANET, ERC and NSRF, European Union;
IN2P3-CNRS, CEA-DSM/IRFU, France; GNSF, Georgia; BMBF, DFG, HGF, MPG and AvH
Foundation, Germany; GSRT and NSRF, Greece; ISF, MINERVA, GIF, I-CORE and Benoziyo Center,
Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO,
Netherlands; BRF and RCN, Norway; MNiSW and NCN, Poland; GRICES and FCT, Portugal; MNE/IFA, Romania; MES of Russia and ROSATOM, Russian Federation; JINR; MSTD,
Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa;
MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SER, SNSF and Cantons of
Bern and Geneva, Switzerland; NSC, Taiwan; TAEK, Turkey; STFC, the Royal
Society and Leverhulme Trust, United Kingdom; DOE and NSF, United States of
America.

The crucial computing support from all WLCG partners is acknowledged
gratefully, in particular from CERN and the ATLAS Tier-1 facilities at
TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France),
KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain),
ASGC (Taiwan), RAL (UK) and BNL (USA) and in the Tier-2 facilities
worldwide.

%----------------------------------------------


